Analyzing Societal Impact of COVID-19: A Study During the Early Days of the Pandemic

In this paper, we collect and study Twitter communications to understand the societal impact of COVID-19 in the United States during the early days of the pandemic. With infections soaring rapidly, users took to Twitter asking people to self isolate and quarantine themselves. Users also demanded closure of schools, bars, and restaurants as well as lockdown of cities and states. We methodically collect tweets by identifying and tracking trending COVID-related hashtags. We first manually group the hashtags into six main categories, namely, 1) General COVID, 2) Quarantine, 3) Panic Buying, 4) School Closures, 5) Lockdowns, and 6) Frustration and Hope}, and study the temporal evolution of tweets in these hashtags. We conduct a linguistic analysis of words common to all hashtag groups and specific to each hashtag group and identify the chief concerns of people as the pandemic gripped the nation (e.g., exploring bidets as an alternative to toilet paper). We conduct sentiment analysis and our investigation reveals that people reacted positively to school closures and negatively to the lack of availability of essential goods due to panic buying. We adopt a state-of-the-art semantic role labeling approach to identify the action words and then leverage a LSTM-based dependency parsing model to analyze the context of action words (e.g., verb deal is accompanied by nouns such as anxiety, stress, and crisis). Finally, we develop a scalable seeded topic modeling approach to automatically categorize and isolate tweets into hashtag groups and experimentally validate that our topic model provides a grouping similar to our manual grouping. Our study presents a systematic way to construct an aggregated picture of peoples' response to the pandemic and lays the groundwork for future fine-grained linguistic and behavioral analysis.

==> models.tex <==
%!TEX root = main.tex
\vspace{-1mm}
In this section, we provide an overview of {\bf SWaP}, a {\bf S}mart {\bf Wa}ter {\bf P}rediction system that takes as input historical water consumption data and outputs future water consumption predictions. Figure \ref{fig:architecture} shows the different components of our system.  {\bf SWaP} comprises of a data pre-processing component, which pre-processes the water consumption data and a prediction component consisting of the proposed models that takes the pre-processed data to generate the desired predictions. We design two models, a discriminative probabilistic graphical model and a deep learning model for the prediction component  in {\bf SWaP}. Specifically, we design i) sparse Gaussian Conditional Random Fields (GCRFs) and ii) Long Short Term Memory (LSTM) based deep Recurrent Neural Network (RNN) models to successfully encode dependencies in the water consumption data. At time $T$, both models accept an input sequence $X$ = [$x_T$, $x_{T-1}$, ...., $x_{T-n}$], which corresponds to amount of water consumed in the last $n$ time steps and generate predictions $Y$ = [$\hat{y}_{T+1}$, $\hat{y}_{T+2}$, ...., $\hat{y}_{T+k}$] for the next $k$ time steps. We note that the input and output sequences can be of different lengths. 

\subsection{Why Sequence-to-Sequence Models?}

Traditional model-based and statistical approaches (e.g., ARIMA models, filtering techniques)  provide valuable insights into data, and are highly desirable when limited computational resources and data are available to make decisions.  The increase  in computational power, the availability of large amounts of data, and growth in the field of machine learning presents the opportunity to design  data-driven techniques capable of providing superior prediction performance in real-world settings. This provides us the opportunity to explore sequence-to-sequence models that are well suited for time-series data problems requiring mapping input sequences to output sequences. Sequence-to-sequence models possess the ability to predict an entire sequence of data points based on past data, thus being able to predict further into the future. To this end,  we identify sequence-to-sequence probabilistic graphical (i.e., sparse GCRFs) and deep learning  models that have been extensively used for a number of forecasting and prediction tasks \cite{bejarano2019, assem2017urban}.  Both GCRF and deep models elegantly learn and capture non-linear dependencies as the encoded signal passes through the network, thus having a positive impact on prediction.

\begin{figure}[!ht]
    \centering
       \includegraphics[trim={0 1cm 0 8cm},clip,scale=0.3]{Figures/architecture}
       \caption{System Architecture}
  \label{fig:architecture} 
\end{figure}

%bahdanau2014neural, angkvist2014review, venugopalan2015sequence

\input{gcrf}


\subsection{RNN Encoder-Decoder Model}

The temporal dependence between the data instances in a sequence prediction problem make recurrent neural networks (RNNs) an appropriate fit for the problem. An RNN consists of a hidden state $h$ and an output $Y$ that operates on input $X$. At each time step $t$, the hidden state of the RNN is given by,
\begin{align}
\label{eqn:rnn}
h_t = f(h_{t-1}, x_t)
\end{align}
where, $f$ is any non-linear activation function and $1$ $\leq$ $t$ $\leq$ $n$. In our problem, $f$ follows a neural network architecture comprising of a network of nodes organized into sequential hidden layers with each node in a given layer being full connected to every other node in the next successive layer. Each hidden state serves as memory and its output is calculated using the output of the previous hidden state and the input $x_t$ as shown in Equation \ref{eqn:rnn}. Since RNNs are known to suffer from the vanishing or exploding gradient problem \cite{hochreiter1998vanishing} when sigmoid functions are used, our architecture uses LSTM cells that use memory cells to store relevant information needed to learn long range temporal dependencies in the data. We refer the reader to Goodfellow et al. for more details on RNN \cite{goodfellow2016deep}.

We develop an LSTM-based RNN encoder-decoder sequence-to-sequence model as shown in Figure \ref{fig:RNN} \cite{cholearning}.  The architecture of both the encoder and decoder is an RNN. The basic cell in both the encoder and the decoder is an LSTM.  The encoder accepts an input sequence and generates a hidden encoded vector $c$ encapsulating the information for the input sequence. This encoded vector is given as an input to the decoder, which then generates the predictions. The input $X$ is transformed into the output $\hat{Y}$ using the hidden layers and the weight matrices. The  weight matrices essentially capture the information needed to generate the output predictions based on the input data. The LSTM cell used in our model consists of a number of  interconnected gated units. The three gates in an LSTM cell are namely,  the input gate,  the output gate, and the forget gate that lets it handle long-term dependencies.
To prevent prediction of negative water consumption values, a ReLU activation function is used after each decoder output. 


%The LSTM unit with a forget gate is implemented by the following composite functions:
%
%\begin{align}
%f_t &= \sigma_g(W_f X_t + U_f H_{t-1} + b_f) \nonumber \\
%i_t &= \sigma_g(W_i X_t + U_i H_{t-1} + b_i) \nonumber \\
%o_t &= \sigma_g(W_o X_t + U_o h_{t-1} + b_o) \nonumber \\
%c_t &= f_t \cdot c_{t-1} + i_t \cdot \sigma_c(W_c X_t + U_c H_{t-1} + b_c) \nonumber \\
%h_t & = o_t \cdot \sigma_h(c_t) 
%\end{align}

%where, $x_t$ is the input vector to the LSTM unit, $f_t$, $i_t$, and $o_t$ are  the forget gate's activation vector, input gate's activation vector, and output gate's activation vectors, respectively. $H_t$ is the hidden state vector, and $C_t$ is the cell state vector. $W$ and $U$ are weight matrices and $b$ are bias vector parameters that are learned during training. $\sigma_g$ is a sigmoid function and $\sigma_c$ and $\sigma_h$  are \textit{tanh} functions.  

\begin{figure}[!ht]
    \centering
       \includegraphics[width=0.8\linewidth]{Figures/rnnencdec}
       \caption{Encoder-decoder based RNN}
  \label{fig:RNN} 
\end{figure}

\subsubsection{Implementation Details} 
We use TensorFlow\footnote{https://www.tensorflow.org/} for implementing the deep learning models. As mentioned in Section \ref{sec:gcrfimp}, we similarly split the datasets into two parts---the first part consisting of 75\% of the data is used for  training and the remaining 25\% is used for testing. Similar to the GCRF models, we use water consumption of past 24 hours (i.e., $n$ = 24) and predict 12 hours into the future (i.e., $k $ = 12).  These settings ensure that the results from both these models are directly comparable. As deep models are computationally expensive, we train our models on a shared high performance computing cluster available at our university.  Using this cluster, we are able to execute  10  to 15 experiments in parallel. Each experiment is allocated 4 cores and 10 GB of RAM. For the datasets considered in this work, for a particular configuration of parameters, training the deep models (i.e., a single experiment) can take in the order of 1 - 12 hours, which is typical of deep learning models. 

We experiment with different number of stacked layers, different numbers of hidden units in each layer as well as the lengths of the input and output sequences. We observe that depending on the dataset, different parameter configurations provide the best performance. However, we empirically observe that overall 1 stacked layer with 200 hidden units generalizes better across all the buildings. We use a learning rate of 0.01 and train the model for 1000 epochs. At training time, the encoder and decoder are trained jointly using the backpropagation algorithm. We use  unguided training as the training scheme, where the decoder uses previous predicted output value as an input to the next step of the decoder. Unguided training enables the model to better explore the state space, which usually results in superior prediction performance at test time. Additionally, to minimize overfitting, we incorporate L2 regularization in the models. 

In comparison to training, the testing phase of a model takes only a couple of minutes for each experiment. The learned weight values for the different connections in the neural network are used to generate a prediction for the test data instances. 


==> references.tex <==
@inproceedings{wytock2013sparse,
  title={Sparse Gaussian conditional random fields: Algorithms, theory, and application to energy forecasting},
  author={Wytock, Matt and Kolter, Zico},
  booktitle={International conference on machine learning},
  pages={1265--1273},
  year={2013}
}

@inproceedings{arjunan2015openban,
  title={OpenBAN: An Open Building ANalytics Middleware for Smart Buildings},
  author={Arjunan, Pandarasamy and Srivastava, Mani and Singh, Amarjeet and Singh, Pushpendra},
  booktitle={proceedings of the 12th EAI International Conference on Mobile and Ubiquitous Systems: Computing, Networking and Services on 12th EAI International Conference on Mobile and Ubiquitous Systems: Computing, Networking and Services},
  pages={70--79},
  year={2015},
  organization={ICST (Institute for Computer Sciences, Social-Informatics and~…}
}

@article{kwon2018connected,
  title={The Connected Shower: Studying Intimate Data in Everyday Life},
  author={Kwon, Hyosun and Fischer, Joel E and Flintham, Martin and Colley, James},
  journal={Proceedings of the ACM on Interactive, Mobile, Wearable and Ubiquitous Technologies},
  volume={2},
  number={4},
  pages={176},
  year={2018},
  publisher={ACM}
}

@inproceedings{assem2017urban,
  title={Urban water flow and water level prediction based on deep learning},
  author={Assem, Haytham and Ghariba, Salem and Makrai, Gabor and Johnston, Paul and Gill, Laurence and Pilla, Francesco},
  booktitle={Joint European Conference on Machine Learning and Knowledge Discovery in Databases},
  pages={317--329},
  year={2017},
  organization={Springer}
}

@inproceedings{giannitrapani2013optimal,
  title={Optimal bidding strategies for wind power producers with meteorological forecasts},
  author={Giannitrapani, Antonio and Paoletti, Simone and Vicino, Antonio and Zarrilli, Donato},
  booktitle={2013 Proceedings of the Conference on Control and its Applications},
  pages={13--20},
  year={2013},
  organization={SIAM}
}

@article{tull2016much,
  title={How Much Water Does Turf Removal Save? Applying Bayesian Structural Time-Series to California Residential Water Demand},
  author={Tull, Christopher and Schmitt, Eric and Atwater, Patrick}
}

@inproceedings{kofinas2016daily,
  title={Daily multivariate forecasting of water demand in a touristic island with the use of artificial neural network and adaptive neuro-fuzzy inference system},
  author={Kofinas, Dimitris and Papageorgiou, Elpiniki and Laspidou, C and Mellios, Nikolaos and Kokkinos, Konstantinos},
  booktitle={2016 International Workshop on Cyber-physical Systems for Smart Water Networks (CySWater)},
  pages={37--42},
  year={2016},
  organization={IEEE}
}

@article{endo2017review,
  title={A review of the current state of research on the water, energy, and food nexus},
  author={Endo, Aiko and Tsurita, Izumi and Burnett, Kimberly and Orencio, Pedcris M},
  journal={Journal of Hydrology: Regional Studies},
  volume={11},
  pages={20--30},
  year={2017},
  publisher={Elsevier}
}

@article{ALI2018104,
title = "Forecasting model for water-energy nexus in Alberta, Canada",
journal = "Water-Energy Nexus",
volume = "1",
number = "2",
pages = "104 - 115",
year = "2018",
issn = "2588-9125",
doi = "https://doi.org/10.1016/j.wen.2018.08.002",
url = "http://www.sciencedirect.com/science/article/pii/S2588912518300122",
author = "Babkir Ali",
keywords = "Alberta, Water forecast, Primary fuels, Electricity generation, Water-energy nexus",
}

@article{RAMBO20173837,
title = "Water-Energy Nexus in Saudi Arabia",
journal = "Energy Procedia",
volume = "105",
pages = "3837 - 3843",
year = "2017",
note = "8th International Conference on Applied Energy, ICAE2016, 8-11 October 2016, Beijing, China",
issn = "1876-6102",
doi = "https://doi.org/10.1016/j.egypro.2017.03.782",
url = "http://www.sciencedirect.com/science/article/pii/S1876610217308500",
author = "Khulood A. Rambo and David M. Warsinger and Santosh J. Shanbhogue and John H. Lienhard V and Ahmed F. Ghoniem",
keywords = "water-energy nexus, oil and gas, electricty production, water use, desalination, Saudi Arabia",
}

@article{mason2018forecasting,
  title={Forecasting energy demand, wind generation and carbon dioxide emissions in Ireland using evolutionary neural networks},
  author={Mason, Karl and Duggan, Jim and Howley, Enda},
  journal={Energy},
  volume={155},
  pages={705--720},
  year={2018},
  publisher={Elsevier}
}

@article{doi:10.1029/2018WR023205,
author = {Quilty, John and Adamowski, Jan and Boucher, Marie-Amélie},
title = {A Stochastic Data-Driven Ensemble Forecasting Framework for Water Resources: A Case Study Using Ensemble Members Derived From a Database of Deterministic Wavelet-Based Models},
journal = {Water Resources Research},
volume = {55},
number = {1},
pages = {175-202},
keywords = {ensemble forecasting, probabilistic forecasting, stochastic, input variable selection, data driven, wavelets},
doi = {10.1029/2018WR023205},
url = {https://agupubs.onlinelibrary.wiley.com/doi/abs/10.1029/2018WR023205},
eprint = {https://agupubs.onlinelibrary.wiley.com/doi/pdf/10.1029/2018WR023205},
year = {2019}
}

@inproceedings{jagarlamudi2012incorporating,
  title={Incorporating lexical priors into topic models},
  author={Jagarlamudi, Jagadeesh and Daum{\'e} III, Hal and Udupa, Raghavendra},
  booktitle={Proceedings of the Conference of the European Chapter of the Association for Computational Linguistics (EACL)},
  year={2012}
}
